OpenGAN: Open-Set Recognition via Open Data Generation

Real-world machine learning systems need to analyze test data that may differ from training data. In K-way classification, this is crisply formulated as open-set recognition, core to which is the ability to discriminate open-set data outside the K closed-set classes. Two conceptually elegant ideas for open-set discrimination are: 1) discriminatively learning an open-vs-closed binary discriminator by exploiting some outlier data as the open-set, and 2) unsupervised learning the closed-set data distribution with a GAN, using its discriminator as the open-set likelihood function. However, the former generalizes poorly to diverse open test data due to overfitting to the training outliers, which are unlikely to exhaustively span the open-world. The latter does not work well, presumably due to the instable training of GANs. Motivated by the above, we propose OpenGAN, which addresses the limitation of each approach by combining them with several technical insights. First, we show that a carefully selected GAN-discriminator on some real outlier data already achieves the state-of-the-art. Second, we augment the available set of real open training examples with adversarially synthesized "fake" data. Third and most importantly, we build the discriminator over the features computed by the closed-world K-way networks. This allows OpenGAN to be implemented via a lightweight discriminator head built on top of an existing K-way network. Extensive experiments show that OpenGAN significantly outperforms prior open-set methods.

==> figure/nbPixels.tex <==
\definecolor{unlabeled}           {RGB}{  0,  0,  0}
\definecolor{ego vehicle}         {RGB}{  0,  0,  0}
\definecolor{rectification border}{RGB}{  0,  0,  0}
\definecolor{out of roi}          {RGB}{  0,  0,  0}
\definecolor{static}              {RGB}{  0,  0,  0}
\definecolor{dynamic}             {RGB}{111, 74,  0}
\definecolor{ground}              {RGB}{ 81,  0, 81}
\definecolor{road}                {RGB}{128, 64,128}
\definecolor{sidewalk}            {RGB}{244, 35,232}
\definecolor{parking}             {RGB}{250,170,160}
\definecolor{rail track}          {RGB}{230,150,140}
\definecolor{building}            {RGB}{ 70, 70, 70}
\definecolor{wall}                {RGB}{102,102,156}
\definecolor{fence}               {RGB}{190,153,153}
\definecolor{guard rail}          {RGB}{180,165,180}
\definecolor{bridge}              {RGB}{150,100,100}
\definecolor{tunnel}              {RGB}{150,120, 90}
\definecolor{pole}                {RGB}{153,153,153}
\definecolor{pole group}          {RGB}{153,153,153}
\definecolor{traffic light}       {RGB}{250,170, 30}
\definecolor{traffic sign}        {RGB}{220,220,  0}
\definecolor{vegetation}          {RGB}{107,142, 35}
\definecolor{terrain}             {RGB}{152,251,152}
\definecolor{sky}                 {RGB}{ 70,130,180}
\definecolor{person}              {RGB}{220, 20, 60}
\definecolor{rider}               {RGB}{255,  0,  0}
\definecolor{car}                 {RGB}{  0,  0,142}
\definecolor{truck}               {RGB}{  0,  0, 70}
\definecolor{bus}                 {RGB}{  0, 60,100}
\definecolor{caravan}             {RGB}{  0,  0, 90}
\definecolor{trailer}             {RGB}{  0,  0,110}
\definecolor{train}               {RGB}{  0, 80,100}
\definecolor{motorcycle}          {RGB}{  0,  0,230}
\definecolor{bicycle}             {RGB}{119, 11, 32}
\definecolor{license plate}       {RGB}{  0,  0,142}




\newcommand{\fnn}[1]{$\scriptstyle^{#1}$}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\tiny]
\begin{axis}[
        ybar,
        bar  width=0.2cm,
        ymode=log,
        width=0.95\textwidth,
        height=5.5cm,
        xmin=-0.2,
        xmax=32, %38.2,
        ymin=7e5,
        ymax=2.5e10,
        ylabel={number of pixels},
        y label style={at={(-0.065,0.5)}, font=\footnotesize},
        xtick=\empty,
        %xtick={2.5,8.5,13.5,19.5,25,28.5,32.5,36},
        %minor xtick={0,5,12,15,24,26,31,34,38},
        %xticklabels = {
%            flat,
%            construction,
%            nature,
%            vehicle,
%            sky,
%            object,
%            human,
%            void,
%        },
        %major x tick style = {opacity=0},
        %minor x tick num = 1,
        %xtick pos=left,
        ymajorgrids=true,
        every node near coord/.append style={
                anchor=west,
                rotate=90,
                font=\scriptsize,
        }
        ]






% flat
\addplot[bar shift=0pt,draw=road,          fill opacity=0.9,fill=road!80!white           , nodes near coords=road ] plot coordinates{ ( 1,     3488951404  ) };
\addplot[bar shift=0pt,draw=building,      fill opacity=0.8,fill=building!80!white       , nodes near coords=build.               ] plot coordinates{ ( 2,     2035086662  ) };
\addplot[bar shift=0pt,draw=vegetation,    fill opacity=0.8,fill=vegetation!80!white     , nodes near coords=veget.               ] plot coordinates{ ( 3,    1538899715  ) };
\addplot[bar shift=0pt,draw=car,           fill opacity=0.8,fill=car!80!white            , nodes near coords=car] plot coordinates{ ( 4,    682420739   ) };
\addplot[bar shift=0pt,draw=sidewalk,      fill opacity=0.8,fill=sidewalk!80!white       , nodes near coords=sidewalk             ] plot coordinates{ ( 5,     520629811   ) };
% sky 
\addplot[bar shift=0pt,draw=sky,           fill opacity=0.8,fill=sky!80!white            , nodes near coords=sky                  ] plot coordinates{ ( 6,    367249493   ) };
\addplot[bar shift=0pt,draw=pole,          fill opacity=0.8,fill=pole!80!white           , nodes near coords=pole                 ] plot coordinates{ ( 7,    116436623   ) };
\addplot[bar shift=0pt,draw=person,        fill opacity=0.8,fill=person!80!white         , nodes near coords=person] plot coordinates{ ( 8,    113919774   ) };
% nature
\addplot[bar shift=0pt,draw=terrain,       fill opacity=0.8,fill=terrain!80!white        , nodes near coords=terrain              ] plot coordinates{ ( 9,    106932536   ) };
% construction
\addplot[bar shift=0pt,draw=fence,         fill opacity=0.8,fill=fence!80!white          , nodes near coords=fence                ] plot coordinates{ ( 10,     71401075    ) };
\addplot[bar shift=0pt,draw=wall,          fill opacity=0.8,fill=wall!80!white           , nodes near coords=wall                 ] plot coordinates{ ( 11,     60820433    ) };
% object
\addplot[bar shift=0pt,draw=traffic sign,  fill opacity=0.8,fill=traffic sign!80!white   , nodes near coords=traffic sign         ] plot coordinates{ ( 12,    51867269    ) };
% vehicle
\addplot[bar shift=0pt,draw=bicycle,       fill opacity=0.8,fill=bicycle!80!white        , nodes near coords=bicycle       ] plot coordinates{ ( 13,    40121126    ) };
\addplot[bar shift=0pt,draw=bus,           fill opacity=0.8,fill=bus!80!white            , nodes near coords=bus           ] plot coordinates{ ( 14,    32155223    ) };
\addplot[bar shift=0pt,draw=truck,         fill opacity=0.8,fill=truck!80!white          , nodes near coords=truck        ] plot coordinates{ ( 15,    24072451    ) };
\addplot[bar shift=0pt,draw=traffic light, fill opacity=0.8,fill=traffic light!80!white  , nodes near coords=traffic light        ] plot coordinates{ ( 16,    19737442    ) };
\addplot[bar shift=0pt,draw=train,         fill opacity=0.8,fill=train!80!white          , nodes near coords=train         ] plot coordinates{ ( 17,    18813992    ) };
% human
\addplot[bar shift=0pt,draw=rider,         fill opacity=0.8,fill=rider!80!white          , nodes near coords=rider        ] plot coordinates{ ( 18,    14651945    ) };
\addplot[bar shift=0pt,draw=motorcycle,    fill opacity=0.8,fill=motorcycle!80!white     , nodes near coords=motorcycle    ] plot coordinates{ ( 19,    8933989     ) };





% Void                                                                                                                                                                        %
\addplot[bar shift=0pt,draw=static,        fill opacity=0.8,fill=static!80!white         , nodes near coords=
\textcolor{darkred}{\bf static}] plot coordinates{ ( 21,    138567142   ) };
\addplot[bar shift=0pt,draw=ground,        fill opacity=0.8,fill=ground!80!white         , nodes near coords=\textcolor{darkred}{\bf ground}] plot coordinates{ ( 22,    121870792   ) };
\addplot[bar shift=0pt,draw=parking,       fill opacity=0.8,fill=parking!80!white        , nodes near coords=\textcolor{darkred}{\bf parking}] plot coordinates{ ( 23,     54936950    ) };
\addplot[bar shift=0pt,draw=dynamic,       fill opacity=0.8,fill=dynamic!80!white        , nodes near coords=\textcolor{darkred}{\bf dynamic}] plot coordinates{ ( 24,    31219463    ) };
\addplot[bar shift=0pt,draw=bridge,        fill opacity=0.8,fill=bridge!80!white         , nodes near coords=\textcolor{darkred}{\bf bridge}] plot coordinates{ ( 25,     21789831    ) };
\addplot[bar shift=0pt,draw=rail track,    fill opacity=0.8,fill=rail track!80!white     , nodes near coords=\textcolor{darkred}{\bf rail track}] plot coordinates{ ( 26,     13301541    ) };
\addplot[bar shift=0pt,draw=tunnel,        fill opacity=0.8,fill=tunnel!80!white         , nodes near coords=\textcolor{darkred}{\bf tunnel}] plot coordinates{ ( 27,    3709525     ) };
\addplot[bar shift=0pt,draw=caravan,       fill opacity=0.8,fill=caravan!80!white        , nodes near coords=\textcolor{darkred}{\bf caravan}] plot coordinates{ ( 28,    3346870     ) };
\addplot[bar shift=0pt,draw=trailer,       fill opacity=0.8,fill=trailer!80!white        , nodes near coords=\textcolor{darkred}{\bf trailer}] plot coordinates{ ( 29,    2476788     ) };
\addplot[bar shift=0pt,draw=guard rail,    fill opacity=0.8,fill=guard rail!80!white     , nodes near coords=\textcolor{darkred}{\bf guard rail}] plot coordinates{ ( 30,    962778      ) };
\addplot[bar shift=0pt,draw=pole group,    fill opacity=0.8,fill=pole group!80!white     , nodes near
coords= \textcolor{darkred}{\bf pole group}] plot coordinates{ ( 31,    727994      ) };

\node at (axis cs:10,1.3e10) [draw=none,anchor=north west,font=\scriptsize] {\textcolor{darkred}{\bf ``void'' pixels not used for training}};


%\node at (axis cs:25.5,3e10) [draw=none,anchor=north west,font=\scriptsize] {\fnn{1} instance-level annotations are available};
%\node at (axis cs:25.5,1.3e10) [draw=none,anchor=north west,font=\scriptsize] {\fnn{2} ignored for evaluation};

\end{axis}
\end{tikzpicture}


